GraphZip: Dictionary-based Compression for Mining Graph Streams

A massive amount of data generated today on platforms such as social networks, telecommunication networks, and the internet in general can be represented as graph streams. Activity in a network's underlying graph generates a sequence of edges in the form of a stream; for example, a social network may generate a graph stream based on the interactions (edges) between different users (nodes) over time. While many graph mining algorithms have already been developed for analyzing relatively small graphs, graphs that begin to approach the size of real-world networks stress the limitations of such methods due to their dynamic nature and the substantial number of nodes and connections involved. In this paper we present GraphZip, a scalable method for mining interesting patterns in graph streams. GraphZip is inspired by the Lempel-Ziv (LZ) class of compression algorithms, and uses a novel dictionary-based compression approach in conjunction with the minimum description length principle to discover maximally-compressing patterns in a graph stream. We experimentally show that GraphZip is able to retrieve complex and insightful patterns from large real-world graphs and artificially-generated graphs with ground truth patterns. Additionally, our results demonstrate that GraphZip is both highly efficient and highly effective compared to existing state-of-the-art methods for mining graph streams.

==> graphzip-arxiv (2)/sig-conf-body.tex <==
\begingroup
% \normalsize
% \vspace{-0.3em}
\section{Introduction}
% Why graphs are important
% Static vs dynamic graphs, why `streaming'
Graphs are used to represent data across a wide spectrum of areas, from computational chemistry %\cite{chem-compound-analysis} 
to social network analysis.
% (?) Talk about what's actually 'mined', FSM etc
%Many graphs that are the target of are  Graph streams are a natural way to represent 
%As advancements in computing allow for the collection and storage of increasingly large datasets, it is important that we develop algorithms capable of efficiently processing the data we collect.
Graph mining is an active 
%and long-standing 
area of research, and there are numerous methods for mining smaller graphs (several thousand edges), but many of these systems are unable to scale to real-world graphs (e.g., social networks) with millions or even billions of edges. %Additionally, many of . 
Conventional graph mining algorithms assume a complete static graph as input, however many real-world graphs are often too large to hold in main memory. %(the Facebook graph has over 400 billion edges \cite{ChingFB}). 
Additionally, many real-world graphs of interest are dynamic and actively growing - Facebook, for example, records over 300 new users per minute and has a social graph with more than 400 billion edges  \cite{ChingFB}. 
%, and Twitter reports over 350,000 tweets per minute. 
While it is possible to utilize conventional graph mining systems on dynamic graphs by processing static `snapshots' of the graph at various points in time, 
%Many improvements have been made to existing approaches in the non-streaming domain
%, yet even for graph mining systems that can scale to handle the sheer size of larger graphs, 
in many cases the underlying data the graph represents changes at a rate so fast that attempting to analyze the data using such methods is futile.
%methods designed for static graphs is futile.

% What is 'streaming'
In cases where the graph in question is inherently dynamic, we can instead treat the graph as a sequential stream of edges representing continuous updates to the graph's overall structure. 
%which can be continuously fed as input to a graph mining system designed to take stream data. 
For example, given a graph modeling friendships (edges) between users (nodes) in a social network, we can consider all new or updated relationships during a set time interval (e.g., 1 hour) a set of edges from time $t_i$ to $t_{i+1}$. The graph mining system then processes the sequential edge sets at every interval, as opposed to attempting to read the entire graph at once. Processing large graphs in a streaming fashion drastically reduces the system's memory requirements (since only small portions of the graph are seen at a time) and enables processing of large, dynamic real-world datasets. 
%that challenge conventional methods. 
However, deploying a streaming model for real-time data analysis also imposes strict constraints: the system has a limited time window to process each set of edges, and edges can only be viewed once before they are replaced in memory by those in the next set. %Consequently, classically `hard' graph mining problems are often considered even harder in the streaming setting. XXX % TODO correct implication?

% TODO needs better transition from prev. segment
% Compression and MDL
% What KIND of mining is actually done (FSM, clique detection, etc)
Many graph mining algorithms aim to identify interesting patterns within an input graph. Various algorithms use different metrics to quantify how `interesting' a pattern is: frequent subgraph mining (FSM) focuses on finding all subgraphs that appear in the graph over a certain frequency threshold, whereas problems such as counting motifs or finding maximal cliques in a graph (formalized in \cite{przulj-motifs} and \cite{bron-kerbosch-cliques}, respectively) focus on discovering subgraphs with a specific structure. 

This paper relies on a novel approach to identify interesting patterns in a graph - namely, finding a set of substructures that best compress the graph.
%A novel approach to finding interesting patterns in a graph is to find a set of patterns that best-compress the graph. More %concretely
More precisely, we compress a graph using a pattern (subgraph) $G$ by replacing all instances of $G$ in the graph with a new node $p$ representing $G$
%, and storing a mapping from $p$ to a single copy of $G$
(see figure \ref{fig:compress}). The reduction in size of the overall graph is a measure of the compression afforded by pattern $G$, and we search for patterns that compress the graph to the maximal extent. 
%want to find patterns that maximally compress a graph. 
The same concept is found in certain types of data compression (e.g., LZ78 \cite{lz78}, ZIP) where the compression method looks for recurring patterns or sequences in the data stream, builds a dictionary representing the recurring patterns with shorter binary codes, and then stores the compressed data using only the binary codes and the dictionary. In the context of graphs, a byproduct of this process is that the pattern dictionary contains a set of subgraphs that compress well, and therefore represents an alternative approach for finding interesting (highly-compressing) patterns in a graph stream.

% Contributions
We propose a dictionary-based compression method for graph-
% \clearpage 
% \noindent
based knowledge discovery: \system{\name}. Our approach is designed to efficiently mine graph streams and uncover interesting patterns by finding maximally-compressing substructures. Specifically, our main contributions are as follows:

\begin{enumerate}
\item We propose a new graph mining paradigm based on the LZ class of compression algorithms.
% \item We introduce a new graph mining algorithm, \system{\name}, designed using this paradigm for efficiently processing massive amounts of data from graph streams.
\item Based on this paradigm, we introduce a new graph mining algorithm, \system{\name}, for efficiently processing massive amounts of data from graph streams.
\item We demonstrate the effectiveness and scalability of our method using a variety of openly available synthetic and real-world datasets.
\end{enumerate}

%Quantitatively,
In our experiments, 
we demonstrate that our approach is able to retrieve both complex and insightful patterns from large real-world graphs by utilizing graph streams. 
%Quantitatively, 
In addition, 
% when we compare 
we show that 
our approach is able to successfully mine a large class of varied substructures from artificially-generated graphs with ground truth patterns. 
When we compare 
%In our experiments we also compare 
\system{\name}'s performance with that of several other state-of-the-art graph mining methods, 
we find that 
%and find that 
\system{\name} consistently outperforms state-of-the-art methods on a variety of real-world datasets. % too bold? 

% The \system{\name} system, including all related code and data used for this paper, will be released at time of publication.
The \system{\name} system, including all related code and data used for this paper, are available for download online\footnote{\url{https://github.com/cpacker/graphzip}}.
% The \system{\name} system including all related code and data used for this paper can be found at the project website\footnote{\url{cpacker.github.io/graphzip}}. % TODO change to github pages site for camera-ready?
\endgroup

\begin{figure}
%     \centering
% \includegraphics[width=\columnwidth]
\includegraphics[width=3.2in]{figs-compression_by_sub_500dpi.png}
    \caption{Compression via substitution. Vertices $A$, $B$, and $C$ form a recurring pattern (subgraph) $G$. Substituting the pattern for a single node $P$ representing $G$ reduces the graph's overall size. The reduction in size is a measure of the compression afforded by pattern $P$. %Note that the compression is lossy since edges connecting $E$ and $D$ to different nodes in the original pattern collapse to edges incident on $P$.
    }\label{fig:compress}
\end{figure}

\section{Related Work}
For the purposes of this paper, we classify previous work into two general categories: streaming and non-streaming.
% TODO Keep heuristic v complete or remove to shortern length of related work?
% We also classify graph mining algorithms as complete or heuristic (i.e., approximate): complete algorithms find all solutions that fit a certain set of criteria, while heuristic algorithms have no such guarantee (and as a result are often faster than their complete counterparts). Heuristic algorithms also place fewer limitations on graph input (e.g., labeling can be incomplete), and therefore can be used on a wider range of real-world graphs.

% TODO mention how completeness affects graph input (limitations on types of graphs, etc)

% Complete vs 'Heuristic' comes from another paper... correct terminology? (or just use 'approximate')

%While several methods have already been developed for analyzing smaller graphs, large graphs such as real-world social networks stress the limitations of such methods due to their dynamic nature and the substantial number of nodes and connections involved. 

\subsection{Non-streaming}
Non-streaming graph mining algorithms take as input either a single graph (single graph mining), or multiple smaller graphs (transactional mining).
% Single graph mining is a generalization of transactional mining

% \noindent
\textbf{Transactional mining.}
%%% Transactional mining
%% TODO go back to (Inokuchi et al., 2000)?
%% FSG (ICDM 2001)
\system{FSG} \cite{fsg} is an early approach to finding frequent subgraphs across a set of graphs, and adopts the Apriori algorithm for frequent itemset mining \cite{apriori}. \system{FSG} works by joining two frequent subgraphs to construct candidate subgraphs, then checking the frequency of the new candidates in the graph.
%% gSpan (ICDM 2002)
\system{gSpan} \cite{gspan} uses a `grow-and-store' approach 
%(similar to \system{GraphZip}) 
that extends saved subgraphs to form new ones, an improvement over \system{FSG}'s prohibitively expensive join operation.
%% Margin (TKTD 2010)
\system{Margin} \cite{margin} prunes the search space to find maximal subgraphs only, a narrower and thus easier problem than FSM.
%% CloseGraph (KDD 2003)
\system{CloseGraph} \cite{closegraph} is another method that reduces the problem space by mining only \emph{closed} frequent subgraphs - subgraphs that have strictly smaller support than any existing supergraphs.
%% Leap (SIGMOD 2008)
\system{Leap} \cite{leap} 
%% GraphSig (ICDE 2009)
and \system{GraphSig} \cite{graphsig} are two recent approaches for mining `significant subgraphs' as measured by a probabilistic objective function. By mining a small set of statistically significant subgraphs as opposed to a complete set of frequent subgraphs, \system{Leap} and \system{GraphSig} are able to avoid the problem of exponential search spaces generated by FSM miners with low frequency thresholds.
% TODO CHECK
%All of the transactional mining algorithms mentioned here are complete.

% \noindent
\textbf{Single graph mining.}
%%% Single graph mining
%% SUBDUE (JAIR 1994)
%In the single graph mining space,
\system{SUBDUE} \cite{subdue} is an approximate algorithm based on the branch-and-bound search technique. \system{SUBDUE}, like \system{\name}, uses the Minimum Description Length (MDL) principle \cite{mdl} to mine maximally-compressing patterns in the graph. However, unlike \system{GraphZip}, \system{SUBDUE} 
%is limited to relatively small graphs, and XXX
returns a restrictively small number of patterns regardless of the size of the input graph \cite{grew}. \system{SUBDUE} has been improved in recent years \cite{subdue2-subgen,subdue3,subdue4}, yet the fundamental limitations of the algorithm (in particular the branch-and-bound technique) remain the same.
% how is it different and similar to GraphZip
% similar to \emph{\name} in that it uses the MDL
%% SEuS (DS 2002)
\system{SEuS} \cite{seus} is an approximate method 
%for mining a single large graph 
that creates a compressed representation of the graph by collapsing vertices that share labels. \system{SEuS} however is only effective in cases where the input graph has a small number of unique subgraphs that occur with high frequency, as opposed to when the input graph has a large number of subgraphs that appear with lower frequency. 
%% SiGram (SDM 2004, DMKD Journal 2005)
\system{SiGram} \cite{sigram} is a complete method for finding frequent connected subgraphs 
(complete methods are guaranteed to find all solutions that fit certain constraints such as the minimum frequency threshold, unlike their approximate counterparts). \system{SiGram} adopts a grow-and-store approach similar to \system{gSpan}, but uses the expensive (NP-complete) Maximal Independent Set (MIS) metric for its frequency threshold, leading the system to be comparatively inefficient in practice. Additionally, like \system{SEuS}, \system{SiGram} suffers from a limited domain problem as it is designed specifically to mine sparse, undirected and labeled graphs only. 
%% Grew (ICDM 2004)
\system{Grew} \cite{grew} 
%developed by the same authors as \system{SiGram}, 
is another approximate method for mining frequent connected subgraphs, and is similar to \system{SUBDUE} in that \system{Grew} only discovers a relatively small subset of solutions in the search space. % TODO reword?
%% GraMi
\system{GraMi} \cite{grami} is a state-of-the-art complete method (with an approximate version \system{AGraMi}) that has been shown to be highly-efficient for FSM on a single large graph. However, the size of the input graph is still 
%significantly 
limited since \system{GraMi} requires the entire graph to be held in main memory.
%% Distributed approaches (include?)
\system{Arabesque} \cite{arabesque} is a recent distributed approach built on top of \system{Apache Giraph} \cite{giraph} that can horizontally scale non-streaming algorithms (FSM, clique finding, motif counting, etc.) across multiple servers. However, horizontal scaling can be cost-prohibitive and is only capable of linearly scaling algorithms whose runtimes often grow exponentially with the size of the input graph. %TODO is this true? maybe talk about how linear scaling can be prohibitively expensive for little gain
%doesn't address many of the fundamental algorithmic limitations of non-streaming approaches. % TODO fix sentence: (memory scaling linearly with graph size, etc). % Better way to say that it's for scaling existing non-streaming algorithms as opposed to a new algorithm?
% GERM
\system{GERM} \cite{germ} and the algorithm introduced by Wackersreuther et al. \cite{wackersreuther} can mine frequent subgraphs in dynamic graphs, however both methods require as input snapshots of the entire graph as opposed to incremental updates to the graph via graph streams.

\subsection{Streaming}
%Compared to the non-streaming setting, few methods exist for graph mining in the streaming setting. 
% GraphScope
\system{GraphScope} \cite{graphscope} is a parameter-free streaming method that, like \system{GraphZip} and \system{SUBDUE}, is based on the MDL principle. \system{GraphScope} encodes the graph stream with the objective of minimizing compression cost, in order to determine important change-points in the temporal data. Beyond change-point and community detection however, \system{GraphScope} has limited use for other tasks, e.g. mining interesting subgraphs. Though the model itself is parameter-free, \system{GraphScope} requires the dimensions of the graph (number of source and destination nodes) to be known \emph{a priori}, and thus is unable to mine streams from dynamic graphs that introduce unseen nodes in new edge streams. 
%(i.e., it is strictly offline). 
% Braun 2014
Braun et al. \cite{braun2014} proposed a novel data structure called DSMatrix for mining frequent patterns in dense graph streams, yet similar to \system{GraphScope} their approach requires that the edges and nodes be known beforehand, limiting its real-world applications.
% Aggarwal VLDB 2010
Aggarwal et al. \cite{aggarwalvldb2010} introduced a probabilistic model for mining dense structural patterns in graph streams, however the approximation techniques used lead to the occurrence of both false positives and false negatives in the results set, reducing the method's viability in many real-world settings. 
% XXX Check:
%Additionally, their method restricts the input to edge-disjoint subgraphs. %Aggarwal and Yu \cite{aggarwalsdm2005} TODO.
% Zips
% Zips \cite{zips} is a recent approach that uses the MDL principle to extract highly-compressing patterns from text data streams, .
% StreamFSM
% TODO add details about performance
\system{StreamFSM} \cite{streamfsm}, based on \system{gSpan}, is a recently introduced method for frequent subgraph mining on graph streams, whose performance we compare directly with that of \system{\name} (see section \S 4).
% Other less relevant streaming methods:
% Doulion: Counting number of triangles in a graph stream
% Not specifically for streaming but works well for it
% \system{Doulion} \cite{doulion}
There also exist several systems targeted at more specific graph analysis tasks in the streaming setting: counting triangles \cite{doulion}, outlier \cite{aggarwalicde2011} and hotspot \cite{aggarwalicdm2013} detection, and link prediction \cite{zhaoicde2016}. 
%, and graph synopses for query estimation \cite{gsketch, gmatrix}.
% Summarization (sketch?) techniques (e.g. TCM)
% \cite{tcm}
% Count-Min Sketch
% \cite{countminsketch}
Summarization methods such as \system{TCM} \cite{tcm}, \system{gSketch} \cite{gsketch} and \system{count-min sketch} \cite{countminsketch} focus on constructing sketch synopses from large graph streams that can provide approximate answers to queries about the graph's properties. 
For a detailed survey of state-of-the-art graph stream techniques, see \cite{streamsurvey} (for a more general overview of graph mining algorithms, see \cite{gmsurvey}). % TODO add an additional another streaming method?

\system{\name} can process an infinite stream of edges without requiring details about nodes or edges beforehand, 
%(i.e., it is fully online), 
and has no restrictions on the type of graph being streamed. While \system{\name} is designed specifically for the streaming setting, it draws from ideas such as grow-and-store and the MDL principle originally applied in non-streaming methods. In contrast to summarization methods, \system{\name} returns exact subgraphs extracted from the stream as opposed to approximate results. To the best of our knowledge, \system{\name} is the first graph mining algorithm for %identifying 
mining maximally-compressing subgraphs from a graph stream.
% TODO extend claim? first LZ-inspired etc?

%% Symbol definitions table
\begin{table}
  \caption{Symbol definitions. Note that \batchsize{} and \dictsize{} are the hyperparameters of the \system{\name} algorithm.}
  \label{table:1}
  \begin{tabular}{@{}ll@{}}
    \toprule
    Symbol & Definition\\
%     Sym. & Definition\\
    \midrule
    $G$ & Arbitrary graph\\ 
    $V_G$ & Vertex set of graph G\\ 
    $E_G$ & Edge set of graph G\\ 
    $S$ & Graph stream sequence\\ 
    $S^{(i)}$ & Graph at time $i$ of stream $S$\\ 
%     $B (\equiv S^{(i)})$ & A batch of edges from graph stream\\
    $B$ & A batch of edges from graph stream\\
    % hline
    $P$ & Pattern dictionary\\ 
    $P^{(i)}$ & Pattern (graph) $i$ in dictionary $P$\\
    $V_{P^{(i)}}$ & Vertex (node) set of pattern $P^{(i)}$\\
    \addlinespace[0.2em]
    $E_{P^{(i)}}$ & Edge set of pattern $P^{(i)}$\\
    \addlinespace[0.2em]
    $C_{P^{(i)}}$ & Compression score of pattern $P^{(i)}$\\
    \addlinespace[0.2em]
    $F_{P^{(i)}}$ & Frequency (count) of pattern $P^{(i)}$\\
    \batchsize & Batch size\\ 
    \dictsize  & Size threshold of $P$\\ 
    % \hline
    %$S(.)$  & Subgraph isomorphism function \\ 
    $H(G)$ & Compression scoring function\\
    $I(G, G)$ & Graph isomorphism function\\
    $SI(G, G)$ & Subgraph isomorphism function\\
  \bottomrule
\end{tabular}
\end{table}

\section{Method}

\subsection{Preliminaries}
In this section, we review the fundamental graph theory needed to formulate our approach and formalize the definitions used in the rest of the paper. See table \ref{table:1} for symbol definitions.

% TODO we should formalize the terms pattern vs subgraph vs substructure vs embedding etc
% \noindent 
\textbf{Terminology.} A graph $G$ is composed of a vertex set $V$ which contains all vertices (nodes) $v \in V$, and an edge set $E$ which contains all edges $e \in E$, each of which connects a source vertex to a target vertex. A subgraph $g$ of $G$ is a graph composed of a subset of $G$'s vertices and edges.
% mention undirected vs directed?
% Remove mention of indexes if not used elsewhere
All vertices $v \in V$ and edges $e \in E$ have a unique \emph{index} which refers to its internal location in the edge or vertex list (e.g., $v_1$ in $V = \{v_1, v_2, v_3\}$ has index $0$, $v_2$ has index 1, etc.). In a vertex-labeled graph, there exists a one-to-one (i.e., unique) mapping from each vertex to a \emph{label}, and in an edge-labeled graph the same mapping exists for the edge set. The value of labels within a graph is often domain-dependent: e.g., in a social network, vertex labels may correspond to a user type (e.g. `male', `female') while edge labels may correspond to different relationship types (e.g. `friend', `family', etc.).

% \begin{definition}
%   If $z$ is irrational, then by $e^z$ we mean the
%   unique number that has
%   logarithm $z$:
%   \begin{displaymath}
%     \log e^z = z.
%   \end{displaymath}
% \end{definition}

% Should these be the fully formal definitions?
% i.e. "a mapping function f:V(G_1) -> V(G_2)" etc
% What about a small figure? Wrong tier audience?
\begin{definition} 
\emph{Isomorphism}: 
Two graphs $G_1$ and $G_2$ are isomorphic (denoted by $G_1 \simeq G_2$) if there is a one-to-one mapping between the edges and vertices of $G_1$ and $G_2$. That is, each vertex $v$ in $G_1$ is mapped to a unique vertex $u$ in $G_2$, the two of which must share the same edges, i.e., be adjacent to the same vertices (if the graph is labeled, the vertices and edges must also share the same labels). 
% This is equivalent to $G_1$ and $G_2$ sharing the same structure.
$G_1 \simeq G_2$ is equivalent to $G_1$ and $G_2$ sharing the same structure.
\end{definition}

\begin{definition}
\emph{Subgraph isomorphism}:
Graph $G_1$ is considered a subgraph isomorphism of graph $G_2$ if it is an isomorphism of some subgraph $g_2$ of $G_2$. The actual instance of $g_2$ is called an \emph{embedding} of $G_1$ in $G_2$. The subgraph isomorphism problem is a generalization of the graph isomorphism problem, and is known to be NP-complete \cite{subiso-npcomplete} (unlike the graph isomorphism problem, the complexity of which is undetermined). Despite the problem's complexity, many graph mining algorithms make heavy use of subgraph isomorphism checks for graph matching, and accordingly several optimizations have been made in the past decade which have significantly improved the efficiency of isomorphism (or subgraph isomorphism) checks in practice. % too much implication of cause->effect?
\end{definition}

\begin{definition}
\emph{Graph stream:}
A graph stream $S$ can be represented as a chronological sequence of edges drawn from a graph. %a sequence of edges 
%$G^{(i)}$ 
%that form incomplete pieces of the complete graph $G$ that the stream is generated from.
%from an initial time point $t$ to time point $t+n$.
\begin{displaymath}
%S = \{ e^{(t)}, e^{(t+1)}, e^{(t+2)}, ... , e^{(t+n)} \}
S = \{ e_{(1)}, e_{(2)}, e_{(3)}, ... , e_{(n)} \}
\end{displaymath}
%If each edge is associated with a time-stamp, then we can process the graph stream by considering all edges from time $t$ to $t+n$ as a single (possibly disconnected) graph stream object.  
We can process the graph stream by segmenting the stream into distinct sets 
%(or `batches') 
of edges, each set forming a single (possibly disconnected) graph stream object. 
%Individual graph stream objects can be represented as sets of edges (i.e. disconnected graphs) that form incomplete pieces of the complete graph $G$ that the stream is generated from. 
% \begin{displaymath}
% %S = \{ e^{(t)}, e^{(t+1)}, e^{(t+2)}, ... , e^{(t+n)} \}
% S = \{ G^{(1)}, G^{(2)}, G^{(3)}, ... , G^{(n)} \}
% \end{displaymath}
In the case of a dynamic graph,  
%(e.g., an active social network),
updates to the graph can be viewed as new stream objects. %An example graph stream would be TODO: $t = 1$ hour. 
In the rest of the paper we also refer to graph stream objects as \emph{batches}, where \emph{batch size} refers to the size of the stream object's edge set (i.e., the number of edges in the batch).
\end{definition}


\subsection{Problem Formulation}
% TODO fill in more, possible expand on MDL here

Given a graph stream and a compression scoring function $H$, our objective function equates to maximizing the cumulative compression score of the entire pattern dictionary $P$:
\begin{equation} \label{e.problem}
	f(G,H) = \argmax_P \sum_i H(P^{(i)})
\end{equation}

The direct approach to solving for $f$ would require enumerating over all possible subgraphs of $G$, a computationally intractable task in most real-world scenarios since it would require storing the entirety of the graph stream, in addition to computing subgraph isomorphism checks over the entire graph. Therefore, we employ a heuristic algorithm to approximate such a solution.

% TODO reorganize + match symbols to definition table
% \newlength{\textfloatsepsave} \setlength{\textfloatsepsave}{\textfloatsep} 
% \setlength{\textfloatsep}{-5pt}
\begin{algorithm}[t!]
\caption{GraphZip}
\label{alg:graphzip}
% {\fontsize{10}{5}
\begin{algorithmic}[1]
%\REQUIRE{Input: $P:=T:=\{ \{1\},\ldots,\{d\}$\}}
%\RETURN{Output: $P:=T:=\{ \{1\},\ldots,\{d\}$\}}
\STATE{Initialize $P$}
\WHILE{edges remain in stream}
	\STATE\label{line3}{Construct graph $B$ using \batchsize{} edges}
	\FOR{\textbf{each} graph $p$ in $P$}
		\STATE{$E$ $\gets$ subgraph isomorphisms of $p$ in $B$}
        \FOR{\textbf{each} graph $g$ in $E$}
        	\STATE{$g' \gets g.copy()$}
            \FOR{\textbf{each} $e$ in $E_g$}
                \IF{$e$ not in $p$}
                    \STATE{Extend $g'$ by new edge $e$}
                \ELSE
                	\STATE{Add internal edge $e$ to $g'$}
                \ENDIF                
            \ENDFOR
            \STATE{Mark each extended edge $e \in B$ as used}
            \IF{$g' \neq g$}
            	\STATE{Add $g'$ to $P$}
            \ENDIF
        \ENDFOR
	\ENDFOR
    \STATE{$R \gets$ remaining unused edges in $B$}
    \STATE{Add edges in $R$ as single-edge patterns to $P$}
\ENDWHILE
\RETURN $P$
\end{algorithmic}
% }
\end{algorithm}
% \setlength{\textfloatsep}{\textfloatsepsave}

\subsection{The \system{\name} Algorithm}
\system{\name} is a highly-scalable method for discovering interesting patterns in a massive graph. Inspired by dictionary-based file compression, \system{\name} builds a dictionary of highly-compressing patterns by counting previously seen patterns in the graph stream and saving new patterns that extend from old ones. The resulting dictionary contains highly-compressing patterns from the given graph stream, which can be used directly or fed into a separate non-streaming algorithm (e.g., a maximal-clique finder). 
%\system{\name} uses this pattern dictionary as a \emph{summarization} state, ... 
While \system{\name} is designed specifically with graph streams in mind, 
%(datasets so large and fast-growing where fitting the graph in main memory is unfeasible)
the algorithm can be easily applied to smaller static graphs without modification: 
%if \system{\name} is given a single graph file, it partitions the edges in the graph into $n \geq 1$ edge sets: 
if \system{\name} is given as input a single graph it will automatically partition it into batches of size \batchsize{} and process the graph as a stream. If the total number of edges in the graph (or number of edges remaining after $n$ iterations) is less than \batchsize{}, \system{\name} will process the graph as a single batch. This flexibility between input types allows us to compare \system{\name} directly with non-streaming methods.

\begin{figure}[t]
\includegraphics[width=\columnwidth]{figs-graphzip_algorithm.pdf}
\caption{A simplified illustration of the \system{\name} algorithm. In dictionary $P$, blue indicates a new pattern, orange indicates a matched pattern extending to a new pattern, and green indicates a non-repeated pattern. After processing $S^{(1)}$, $P$ contains only single edge patterns. $A$-$B$, $C$-$A$, and $D$-$C$ are embedded in $S^{(2)}$, so they are extended as new patterns in $P$. $C$-$A$-$B$ is embedded in $S^{(3)}$, and is extended with an internal edge as a new pattern, along with the remaining edge $D$-$B$.}
\label{fig:algorithm}
% \vspace{1.3mm}
% \vspace{3mm}
\end{figure}


The general procedure of \system{\name} is illustrated in figure 2. \system{\name} is initialized with an empty dictionary $P$ with max size \dictsize{} (provided by the user), which maps graphs to their frequency (count) and compression score.  \system{\name} collects arriving edges from the graph stream into batches of size \batchsize{} (also provided by the user), and runs the $compress$ procedure on each batch $B$: if a pattern $p$ from the dictionary is embedded in $B$, \system{\name} increments the frequency of the pattern in the dictionary and recomputes its compression score. Additionally, for each instance $i$ of pattern $p$ embedded in batch $B$, \system{\name} extends $p$ by one edge length, tagging each of the edges from $B$ used to extend $p$. The new edges used to extend $p$ are the edges incident on $i$ that exist in batch $B$ but not in pattern $p$. \system{\name} then adds the new extended pattern to $P$. After $P$ has been updated with all the extended patterns, the remaining untagged edges in $B$ are added as single-edge patterns to $P$. 
Our current reference implementation supports both undirected and directed edges, but not hyper-edges or self-loops. However, these limitations are implementation specific rather than inherent to the algorithm. Additionally, both representational variants can be converted to simple edges (a node and two edges).

% TODO recheck extension method in python code to match
% TODO mention how using #edges for graph size is standard
If the dictionary exceeds size 2\dictsize{}, the dictionary is sorted according to the compression scores and trimmed to \dictsize{}. A pattern's compression score is computed as follows:
\begin{equation} \label{e.scorefunction}
	H(P^{(i)}) = (|E_{P^{(i)}}| - 1) \times (F_{P^{(i)}} - 1)
\end{equation}
This equates a pattern's compressibility to a product of its size and frequency. We use $(F_{P^{(i)}} - 1)$ so that a pattern with a frequency of $1$ has a compression score of $0$, since a pattern that only appears once affords no real compression  to the overall graph. The same offset is applied to the pattern size in $(|E_{P^{(i)}}| - 1)$ to reduce the weighting of single-edge patterns. 
Due to the fact that overlapping instances of a pattern in a batch are counted independently, it is possible that \system{\name} will overestimate the compression value of large structures with many homomorphisms. 

Note that the compression method used is intrinsically lossy, since \system{\name} does not retain information on how each of the instances are connected to the rest of the graph. The main focus of our work is knowledge discovery in graph streams, so lossy compression is an appropriate trade-off for decreased complexity and increased performance. More work is necessary to make \system{\name} lossless, for example in the case where it is necessary to fully reconstruct the original graph from the pattern dictionary.

See algorithm \ref{alg:graphzip} for pseudo-code, and the online repository for a reference implementation.
% \phantom{spacer}
% TODO UPDATE WITH RELEASE OF CODE, and the project website for the actual implementation.
% TODO talk about how parameters change the size of patterns mined?

% \begin{figure}[t]
% \setlength{\belowcaptionskip}{-10pt}
% \end{figure}
\subsection{Scalability}
Speed and memory usage are critical properties of graph mining algorithms designed to mine large real-world graphs. A deployed graph mining system should be able to keep up with the flow of data in the dynamic graph setting,
%(and preferably run in a reasonable amount of time in the static graph setting)
%, and the system needs an optimized way of summarizing in memory a possibly infinite graph stream. 
%while summarizing in memory a possibly infinite graph stream in an optimized fashion. 
while summarizing a possibly infinite graph stream in memory. 
Memory usage in \system{\name} is directly bounded by the maximum dictionary size (\dictsize{}), 
%and grows at maximum capacity as the graph objects stored in the dictionary grow larger, however the size of the stored graphs
and is indirectly bounded by the batch size (\batchsize{}), since the patterns within the dictionary cannot grow larger than the batch size (no subgraph isomorphisms of the pattern in the batch will exist). 
% TODO probably should mention how subiso checks get slower as pattern in dictionary get larger... or do they?
% Should subiso checks be fast in the case of a NO answer (when pattern we're searching for in batch is very large?) 
Both parameters \dictsize{} and \batchsize{} can be modified to maximize performance given certain hardware limitations.

% include profiling breakdown as chart?
The bulk of the computation in the \system{\name} algorithm happens while checking for embeddings of pattern $p$ in batch $B$ (\emph{find all subgraph isomorphisms of $p$ in $B$}). Note that because each entry in the pattern dictionary is unique, none of the subgraph isomorphism checks are contingent on each other, and thus the loop can be na\"{\i}vely parallelized across an arbitrary number of cores. This allows for large performance gains and means that an increase in dictionary size can be scaled linearly with an increase in cores. 
% terminology?
Even without parallelization of the subgraph isomorphism checks, \system{\name} is still faster than other state-of-the-art graph mining systems (as described in section \S 4). See section \S A for a formal runtime analysis.
% TODO include pie-chart breakdown of runtime via profiler

%%% Figures
%% CPU Utilization by method on example dataset (from python profiling module)
%% Memory usage breakdown (more difficult to get data for)
%% 

% \begin{tabular}{@{}ccccc@{}} \toprule
% \multicolumn{2}{c}{Item} \\ \cmidrule(r){1-2}
% Animal & Description & Price (\$)\\ \midrule
% Gnat & per gram & 13.65 \\
% & each & 0.01 \\
% Gnu & stuffed & 92.50 \\
% Emu & stuffed & 33.33 \\
% Armadillo & frozen & 8.99 \\ \bottomrule
% \end{tabular}

\section{Experimental Evaluation}
There are two main questions we focus on when evaluating our 
%graph mining 
algorithm: does it generate objectively and subjectively good results (i.e. correct and interesting results, respectively), and does it generate them in a reasonable amount of time? To answer these questions we test \system{\name} on an extensive suite of synthetic and real datasets ranging from a few thousand to several million nodes and edges (see table \ref{tab:datasets}). Using these datasets, we benchmark \system{\name} against three state-of-the-art, openly available graph mining systems: \system{SUBDUE}\footnote{\url{http://ailab.wsu.edu/subdue}}, \system{GraMi}\footnote{\url{https://github.com/ehab-abdelhamid/GraMi}}, and \system{StreamFSM}\footnote{\url{https://github.com/rayabhik83/StreamFSM}}.  
%We chose \system{SUBDUE} because it is a TODO, \system{GraMi} beca, and \system{StreamFSM}.
%each with source code available online (see footnotes). 
Because there is no directly comparable method to \system{\name} for mining maximally-compressing patterns in graph streams, we instead evaluate \system{\name} against a non-streaming method for mining compressing patterns (\system{SUBDUE}), a non-streaming method for frequent subgraph mining (\system{GraMi}), and a streaming method for frequent subgraph mining (\system{StreamFSM}). Highly-compressing patterns are often both large and frequent, so FSM methods serve as an appropriate comparison to \system{\name}. % in lieu of direct benchmark.

All experiments were run on a compute server configured with an AMD Opteron 6348 processor (2.8 GHz) and 128GB of RAM.

\begin{figure}[t!]
\includegraphics[width=\columnwidth]{figs-graph_classes.pdf}
\caption{We embed different types of graph substructures into our synthetic graphs, and then test to see if they are recovered. Corresponding datasets (from left to right): 3-CLIQ, 4-CLIQ, 4-STAR, 4-PATH, 8-TREE.}\label{fig:groups}
% \vspace{-0.25in}
\end{figure}

%Testing whether the substructures generated by are \emph{correct} (i.e. maximally compressing) is computationally intractable, since it would require this would require enumerating over all .

% \begin{enumerate}
%   \item Does it generate objectively good (i.e. correct) results?
%   \item Does it generate subjectively good (i.e. interesting) results?
%   \item Does it generate the results in a reasonable amount of time?
% \end{enumerate}

\subsection{Synthetic graphs}
To test whether our algorithm outputs \emph{correct} substructures, we utilize a tool called \system{SUBGEN} \cite{subdue2-subgen} to embed ground truth patterns with desired frequencies into an artificially generated graph. This allows us to test whether or not a graph mining system correctly surfaces known patterns we expect to be returned in the result set. Since both \system{\name} and \system{SUBDUE} are designed to mine highly-compressing patterns from a graph, we embed large and frequent (i.e., highly-compressing) patterns in the graph, then record the number of ground truth patterns recovered. Given a set of embedded patterns $E$, and a set of patterns $R$ returned by our graph mining system, an embedded pattern $E^{(i)} \in E$ is considered \emph{matched} if for some returned pattern $R^{(i)} \in R$, $R^{(i)} \simeq E^{(i)}$.
Thus, we calculate the fraction $a$ of embedded patterns recovered using the scoring metric
%using the scoring metric:
\begin{equation} \label{e4.1}
% 	a = \frac{|\{E^{(i)} | E^{(i)} \in E \wedge R^{(i)} \in R \wedge E^{(i)} \simeq R^{(i)}\}|}{|E|}
	a = |\{E^{(i)} | E^{(i)} \in E \wedge R^{(i)} \in R \wedge E^{(i)} \simeq R^{(i)}\}|\ /\ |E|
\end{equation}
% % TODO convert to math equation using symbols
Which is equivalent to
\begin{equation} \label{e4.2}
	%\textit{\small accuracy} = \frac{\textit{\small matched patterns}}{\textit{\small total patterns}}
    \textit{\small accuracy} = {\textit{\small matched patterns } } / { \textit{ \small total patterns}}
\end{equation}
We count a ground truth pattern as \emph{matched} if it is found in \system{\name}'s pattern dictionary after the final batch, or in \system{SUBDUE}'s case, if it is returned directly at the end of the program.
% XXX issues with "precision" vs "recall"

In addition to making the ground truth patterns highly-compressing, we also design the patterns to cover a wide class of fundamental graph patterns, including cliques, paths, stars and trees (see figure \ref{fig:groups}). This allows us to discern if a method has difficulty mining a certain type of structure (e.g., a poorly designed system may have trouble detecting cycles and therefore cliques). The naming scheme for each synthetic graph dataset is \emph{N-TYPE}, where $N$ is the number of vertices in the embedded pattern and \emph{TYPE} is a shorthand of the pattern type (e.g., 3-CLIQ is a graph with embedded 3-cliques). 
All synthetic graphs in table \ref{table:graphzip-subdue-synthetic} are generated with 1000 nodes, 5000 edges, and 20\%, 50\% or 80\% coverage (the percentage of the graph covered by instances of the pattern). %We use a relatively small graph in this case to , 
%XXX More patterns

\begin{table}[t]
  \caption{\system{\name} and \system{SUBDUE} runtime and accuracy on various synthetic graphs. For runtime, lower is better. For \system{SUBDUE}, the `{+}' for runtime indicates the program was terminated after 1000 seconds (no accuracy shown).}
  \label{table:graphzip-subdue-synthetic}
  \begin{tabular}{@{}lccc@{}c@{}cc@{}}
    \toprule
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Cov.} & \multicolumn{2}{c}{Runtime (sec.)} & \phantom{a} & \multicolumn{2}{c}{Accuracy (\%)} \\
    \cmidrule(lr{0em}){3-4} \cmidrule{6-7}
    & (\%) & {\small \system{\name}} & {\small \system{SUBDUE}} & \phantom{abc} & {\small \system{\name}} & {\small \system{SUBDUE}} \\
    \midrule
    \addlinespace[0.5em]
    \multirow{3}{*}{3-CLIQ} 
    & 20 & \textbf{52.25} & 66.68 & & \textbf{100.0} & 89.24 \\
    \addlinespace[-0.2em]
    & 50 & \textbf{3.779} & 22.22 & & \textbf{100.0} & 89.61 \\
	\addlinespace[-0.2em]
    & 80 & \textbf{3.665} & 11.99 & & \textbf{100.0} & 86.61 \\
%     \midrule
	\addlinespace[0.3em]
    \multirow{3}{*}{4-PATH} 
    & 20 & \textbf{45.37} & 58.00 & & \textbf{100.0} & 100.0 \\  
    \addlinespace[-0.2em]
    & 50 & \textbf{3.052} & 18.57 & & \textbf{100.0} & 100.0 \\  
    \addlinespace[-0.2em]
	& 80 & \textbf{2.935} & 10.30 & & \textbf{100.0} & 100.0 \\  
%     \midrule
    \addlinespace[0.3em]
    \multirow{3}{*}{4-STAR}
    & 20 & \textbf{50.70} & 1000{+} & & \textbf{100.0} & - \\
    \addlinespace[-0.2em]
    & 50 & \textbf{4.184} & 1000{+} & & \textbf{100.0} & - \\
    \addlinespace[-0.2em]
    & 80 & \textbf{4.483} & 1000{+} & & \textbf{100.0} & - \\
%     4-SQRE & & \textbf{8.88} & 91.92 & & 39.8 & \textbf{88.7} \\ % XXX
%     4-DIAM & & \textbf{8.88} & 91.92 & & 39.8 & \textbf{88.7} \\ % XXX
%     \multirow{2}{*}{5-STAR}
%     & & \textbf{7.19} & 1000* & & \textbf{100} & - \\ % XXX
% 	\midrule
	\addlinespace[0.3em]
    \multirow{3}{*}{4-CLIQ}
    & 20 & \textbf{68.06} & 1000{+} & & \textbf{100.0} & - \\
    \addlinespace[-0.2em]
    & 50 & \textbf{29.19} & 1000{+} & & \textbf{100.0} & - \\
    \addlinespace[-0.2em]
    & 80 & \textbf{13.92} & 44.78 & & \textbf{100.0} & 89.51 \\
% 	\midrule
	\addlinespace[0.3em]
    \multirow{3}{*}{5-PATH}
    & 20 & \textbf{48.47} & 1000{+} & & \textbf{100.0} & - \\
    \addlinespace[-0.2em]
    & 50 & \textbf{4.461} & 21.30 & & \textbf{100.0} & 99.81 \\
    \addlinespace[-0.2em]
    & 80 & \textbf{4.267} & 24.16 & & \textbf{100.0} & 99.42 \\
%     \multirow{2}{*}{5-STAR}
%     & & \textbf{7.19} & 1000* & & \textbf{100} & - \\ % XXX
% 	\midrule
	\addlinespace[0.3em]
    \multirow{3}{*}{8-TREE}
    & 20 & \textbf{62.68} & 1000{+} & & \textbf{100.0} & - \\
    \addlinespace[-0.2em]
    & 50 & \textbf{10.39} & 1000{+} & & \textbf{99.65} & - \\
    \addlinespace[-0.2em]
    & 80 & \textbf{11.07} & 1000{+} & & \textbf{100.0} & - \\
    \addlinespace[0.1em]
  	\bottomrule
\end{tabular}
% \vspace{-0.1mm}
\end{table}

\subsection{Comparison with \system{SUBDUE}}

Table \ref{table:graphzip-subdue-synthetic} shows the runtime and accuracy (eq. \ref{e4.1}) for \system{\name} and \system{SUBDUE} on the synthetic datasets. \system{\name} is clearly faster than \system{SUBDUE}, taking an order of magnitude less runtime in most experiments. Decreasing the coverage across all pattern types increased the runtime for both systems. 
\system{SUBDUE} is unable to process half of the datasets (including all 4-STAR and 8-TREE experiments) in less than 1000 seconds, while \system{\name} is able to process the same datasets in a fraction of the time with 99-100\% accuracy in all cases.

Among the datasets \system{SUBDUE} is able to process, the greatest difference in accuracy lies in the clique datasets (3-CLIQ and 4-CLIQ), where \system{SUBDUE} misses approximately 10\% of the embedded patterns. 
%For algorithms that implement a grow-and-store approach to pattern mining, cycles can be difficult to detect since it edges that form cycles often already exist is  that a 3-edge cycle pattern (without extra incident edges) will be formed during the extend phase . 
The \system{\name} algorithm contains an explicit edge case to extend internal edges in a pattern with no new vertices, which enables \system{\name} to capture cliques with high accuracy (see algorithm \ref{alg:graphzip} and figure \ref{fig:algorithm}). % TODO show what pattern was actually mostly captured
% Summary of what the synthetic experiments show

Our results indicate a stark difference in efficiency between \system{\name} and \system{SUBDUE}: \system{SUBDUE} is significantly slower than \system{\name} even on relatively small graphs with several thousand edges, and for graphs with certain classes of embedded patterns in them (stars and binary trees are particularly problematic). For this reason, when evaluating \system{\name} with larger real-world graphs we focus on benchmarking against more scalable methods.

% \subsection{Recovered substructures}
% TODO


% \begin{figure}
% \includegraphics[width=\columnwidth]{figures/exp_growth_3.png}
% \caption{\system{\name} vs \system{SUBDUE} runtime on a graphs of varying size embedded with 3-cliques. We vary the number of vertices with the edges to maintain 10\% density. Compared to \system{\name}, SUBDUE's runtime grows exponentially with the size of the graph.}
% \label{fig:subdue-growth}
% \end{figure}


\subsection{Real-world graphs}
We use several large, real-world graph datasets to test the scalability of the \system{\name} algorithm. See table \ref{tab:datasets} for further details. \\
% \emph{Twitter}\footnote{\url{http://socialcomputing.asu.edu/datasets/Twitter}}: The ASU Twitter dataset \cite{asu-twitter} is a graph of who-follows-who on \url{twitter.com}. The graph contains over 11 million nodes and 85 million edges. Each node represents a user, and two users are connected by an edge from the follower to the followee. \\ % TODO add preprocessing step (100 labels, normally distributed) 
\emph{NBER}\footnote{\url{http://www.nber.org/patents}}: NBER \cite{nber} is a graph of all U.S. patents granted (from Jan. 1963 to Dec. 1999) and the citations between them. The graph contains nearly 4 million nodes (patents) and over 16 million edges. Each node (citing patent) has edges to all the patents in its citation section. We added time-stamps to the citation graph prepared by \cite{snap-nber} and removed all withdrawn patents which had missing metadata ($<$ 0.04\% of all edges).\\
% \emph{DBLP}\footnote{\url{http://projects.csail.mit.edu/dnd/DBLP}}: The DBLP dataset is a co-authorship graph of over 1 million authors across more than 10 million publications in computer science. Each node represents an author, and two authors are connected by an (undirected) edge if they co-authored a publication together. As part of pre-processing, we remove all co-authorship data without year information ($<$ 0.2\% of all edges).\\
\emph{HetRec}\footnote{\url{http://grouplens.org/datasets/hetrec-2011}}: The HetRec 2011 MovieLens 2k \cite{hetrec} dataset links movies of the MovieLens 10M\footnote{\url{http://www.grouplens.org}} dataset with information from their IMDb\footnote{\url{http://www.imdb.com}} and Rotten Tomatoes\footnote{\url{http://www.rottentomatoes.com}} pages. We use a version of the dataset arranged by \cite{streamfsm}, in which nodes are labeled as `movie', `actor' or `director'. Edges connect movies to actors and directors: an edge from movie to director is labeled `directed-by', and an edge from movie to actor is labeled `acted-by'. The data spans 98 years, and is split into one graph stream (batch) file per year. \\
% \emph{CiteSeer}\footnote{\url{http://cs.umd.edu/projects/linqs/projects/lbc}}: CiteSeer \cite{citeceer} is a network of over 3000 publications in computer science and more than 4000 citations between them. We use a version of the graph prepared by \cite{grami}: each publication (node) is labeled with one of six computer science sub-fields (AI, IR, etc.), and each citation (edge) is labeled 0-100 based on the similarity of text of the two papers. \\
% The \emph{Higgs} dataset is described in section \S5.
\emph{Higgs}\footnote{\url{https://snap.stanford.edu/data/higgs-twitter.html}}: The \emph{Higgs Twitter Dataset} \cite{higgs} is a collection of 
%57,949 
563,069 interactions (retweets, mentions, and replies) between 
%45,962
304,691 users on Twitter before, during, and after the announcement of the discovery of Higgs boson particle on July 4th, 2012. The Tweets were scraped over the course of one week (168 hours) by filtering tweets for the tags `lhc', `cern', `boson' and `higgs'. 
%We use anonymous user IDs as node labels, and
Edges are labeled using the type of the interaction between the two users (`retweet', `mention', and `reply'), while all nodes share the same `user' label. 


\begin{table}[t]
  \caption{Details of real-world datasets used. The average stream-rate (in edges per second) is calculated by dividing the total number of edges by the time span of the entire graph.
  %\emph{Twitter} has no stream-rate since the edges lack time information.
  }
  \label{tab:datasets}
%   \begin{center}
  \begin{tabular}{@{}lrrrr@{}}
  	\toprule
    Dataset & Vertices & Edges & Labels & Stream-rate  \\
%     \multirow{2}{*}{Dataset} & \multirow{2}{*}{Vertices} & \multirow{2}{*}{Edges} & Streaming  \\
%      &  &  & -rate  \\
    \midrule
%     Twitter & 11,316,811 & 85,331,846 & 100 & N/A  \\
%     Twitter & 11,316,811 & 85,331,846 & 100 & N/A  \\
    NBER & 3,774,218 & 16,512,783 & 418 & $1.4 \times 10^{-2}$ \\
%     DBLP & 1,412,414 & 10,597,380 & 1 & $4.6 \times 10^{-3}$  \\
    Higgs & 304,691 & 563,069 & 4 & $9.3 \times 10^{-1}$  \\
    HetRec & 108,451 & 241,897 & 5 & $7.8 \times 10^{-5}$ \\
%     Higgs & 45,962 & 57,949 & 4 & $5.8 \times 10^{0}$  \\
%     CiteCeer & 3,312 & 4,732 & 6 & N/A  \\
    \bottomrule
  \end{tabular}
%   \end{center}
\end{table}

% \begin{table}
%   \caption{\system{\name} vs \system{SUBDUE} runtime and accuracy on various synthetic graphs. Higher is better. For \system{SUBDUE}, both the 3-star and 7-binary-tree experiments were terminated after 1000 seconds (no accuracy shown).}
%   \label{table:graphzip-subdue-synthetic}
%   \begin{tabular}{ccccc}
%     \toprule
%     \multirow{2}{*}{Dataset} & \multicolumn{2}{c}{Runtime (sec.)} & \multicolumn{2}{c}{Accuracy (\%)} \\
%     \cmidrule(r){2-5}
%     & \system{\name} & \system{SUBDUE} & \system{\name} & \system{SUBDUE} \\
%     \midrule
%     3-CLIQ  & \textbf{8.88} & 91.92 & 39.8 & \textbf{88.7} \\
%     3-PATH  & \textbf{7.19} & 34.46 & \textbf{100} & 100 \\
%     4-PATH  & \textbf{4.84} & 49.07 & \textbf{100} & 99.0 \\
%     3-STAR  & \textbf{7.19} & 1000* & \textbf{100} & - \\
%     7-TREE  & \textbf{14.20} & 1000* & \textbf{100} & - \\
%   	\bottomrule
% \end{tabular}
% \end{table}

% Page-wide figure composed of two big-figs each with two small-figs
\begin{figure*}[t]
\begin{minipage}[t]{0.48\linewidth}

\begin{figure}[H]
\centering

% NBER stream-rate
% \begin{subfigure}[b]{\columnwidth}
% \begin{subfigure}[H]{0.45\linewidth}
\begin{subfigure}[H]{0.47\linewidth}
%     \includegraphics[width=\linewidth]{figures/graphzip_v_grami_streamrate_per_file_nber_lscale.pdf}
    \includegraphics[width=\linewidth]{figs-nber_sr_lscale.pdf}
    \caption{
%     \system{\name} and \system{GraMi} stream-rate on \textit{NBER}.% Higher is better.
    }
    \label{fig:graphzip_grami_sr_nber}
\end{subfigure}\qquad
% NBER runtime
% \begin{subfigure}[H]{0.45\linewidth}
\begin{subfigure}[H]{0.44\linewidth}
    \includegraphics[width=\linewidth]{figs-nber_runtime.pdf}
    \caption{
%     \system{GraphZip} and \system{GraMi} runtime on \textit{NBER}.
    }
    \label{fig:graphzip_grami_rt_nber}
\end{subfigure}
\vspace{-3mm}
\caption[Two numerical solutions]{Stream-rate (a) and runtime (b) of \system{\name} and \system{GraMi} on the \textit{NBER} dataset. \system{GraMi}'s stream-rate decrease significantly near the end, while \system{\name}'s stream-rate remains relatively constant.}
\label{fig:graphzip_grami_nber}
\end{figure}

\end{minipage}%
    \hfill%
\begin{minipage}[t]{0.48\linewidth}

\begin{figure}[H]
\centering

% HetRec stream-rate
% \begin{subfigure}[b]{\columnwidth}
% slightly wider to accommodate for label
\begin{subfigure}[H]{0.47\linewidth}
%     \includegraphics[width=\linewidth]{figures/graphzip_streamrate_nber.pdf}
    \includegraphics[width=\linewidth]{figs-hetrec_sr_lscale.pdf}
    \caption{
    }
    \label{fig:graphzip_streamfsm_sr_hetrec_l}
\end{subfigure}\qquad
% HetRec runtime
\begin{subfigure}[H]{0.44\linewidth}
%     \includegraphics[width=\linewidth]{figures/graphzip_v_grami_runtime_per_file.pdf}
    \includegraphics[width=\linewidth]{figs-hetrec_runtime.pdf}
    \caption{
    }
    \label{fig:graphzip_streamfsm_rt_hetrec_nl}
\end{subfigure}
\vspace{-3mm}
\caption[]{Stream-rate (a) and runtime (b) of \system{\name}, \system{GraMi}, and \system{StreamFSM} on the \textit{HetRec} dataset. Both \system{GraMi} and \system{StreamFSM} experience a massive spike in runtime near iteration 93.}
\label{fig:graphzip_streamfsm_hetrec}
% \vspace{-3mm}
\end{figure}

\end{minipage}%
\vspace{-1.0mm}
\end{figure*}


\begin{figure}
\vspace{2mm}
\centering
% Scatter plots
% \begin{subfigure}[b]{\columnwidth}
\begin{subfigure}[H]{0.45\linewidth}
% \begin{subfigure}[H]{0.47\linewidth}
%     \includegraphics[width=\linewidth]{figures/graphzip_v_grami_streamrate_per_file_nber_lscale.pdf}
    \includegraphics[width=\linewidth]{figs-nber_scatter.pdf}
    \caption{
    }
    \label{fig:graphzip_nber_scat}
\end{subfigure}\qquad
\begin{subfigure}[H]{0.45\linewidth}
% \begin{subfigure}[H]{0.44\linewidth}
    \includegraphics[width=\linewidth]{figs-hetrec_scatter.pdf}
    \caption{
    }
    \label{fig:graphzip_hetrec_scat}
\end{subfigure}
\vspace{-3mm}
\caption[]{Distribution of \system{\name}'s pattern dictionary after 300 iterations on \emph{NBER} (a) and after 98 iterations on \emph{HetRec} (b). The distribution for the larger \emph{NBER} dataset (a) is skewed towards patterns with high frequencies, while the distribution for patterns in \emph{HetRec} (b) is more varied.}
\label{fig:graphzip_scats}
\vspace{-1mm}
\end{figure}

% \begin{figure*}[t]
% \begin{minipage}[t]{0.225\linewidth}
%     \includegraphics[width=\linewidth]{figures/graphzip_v_grami_streamrate_per_file_nber_lscale.pdf}
% %     \captionsetup{justification=raggedright}
%     \caption{
%     \system{GraphZip} stream-rate while processing \textit{NBER}. Higher is better.
%     }
%     \label{fig:graphzip_grami_sr_nber}
% \end{minipage}%
%     \hfill%
% \begin{minipage}[t]{0.225\linewidth}
% 	\centering
%     \includegraphics[width=\linewidth]{figures/graphzip_v_grami_runtime_per_file_nber_lscale.pdf}
%     \caption{\system{GraphZip} and \system{GraMi} runtime on \textit{NBER}.}
%     \label{f2}
% \end{minipage} 
%     \hfill%
% \begin{minipage}[t]{0.225\linewidth}
%     \includegraphics[width=\linewidth]{figures/graphzip_streamrate_nber.pdf}
%     \caption{\system{GraphZip} stream-rate while processing \textit{NBER}.}
%     \label{f1}
% \end{minipage}%
%     \hfill%
% \begin{minipage}[t]{0.225\linewidth}
% 	\centering
%     \includegraphics[width=\linewidth]{figures/graphzip_v_grami_runtime_per_file.pdf}
%     \caption{\system{GraphZip} and \system{GraMi} runtime on \textit{NBER}.}
%     \label{f2}
% \end{minipage} 
% \end{figure*}

\subsection{Comparison with \system{GraMi}}
Despite being designed for mining highly-compressing patterns like \system{\name}, \system{SUBDUE} has clear performance issues that restrict benchmarking it against \system{\name} on large real-world graphs. 
%Since there are few openly available systems for mining patterns from graph streams, we benchmark \system{\name} against 
Therefore we also compare \system{\name} with \system{GraMi}, a state-of-the-art graph mining system for frequent subgraph mining on large static graphs. In contrast to \system{SUBDUE}, \system{GraMi} is efficient enough to process datasets with millions of edges, 
however \system{GraMi}'s relative performance still allows us to motivate the need for graph mining algorithms designed explicitly to handle streaming data.
%from dynamic graphs. 

\system{GraMi} takes as input a single graph file as opposed to a sequence of edges, so in order to simulate mining a dynamic graph with a non-streaming method we append the previous graph with the next set of edges at each iteration, initializing the graph with the first set of edges. Thus, each iteration represents a `snapshot' of the growing graph. Since both methods are paramaterized, we first tune \system{GraMi}'s minimum frequency threshold so that it returns a usable number of non-single edge patterns, then set \system{\name}'s parameters (batch and dictionary size) such that the pattern dictionary resembles the set of subgraphs returned by \system{GraMi}. On \emph{NBER} (figure \ref{fig:graphzip_grami_nber}), we fix \system{GraMi}'s minimum frequency threshold to 1000 which returned a set of subgraphs with a maximum, minimum, and average size of $6$, $1$, and $1.47$ respectively. Running \system{\name} with $\alpha = 5$ and $\theta = 50$ resulted in a pattern dictionary with a maximum, minimum, and average subgraph size of $5$, $1$, and $2.89$ (figure \ref{fig:graphzip_scats} shows the dictionary distributions for both \emph{NBER} and \emph{HetRec}). Since the overall runtime of each model depends significantly on the configuration of the parameters, 
%(e.g., setting \system{GraMi}'s minimum frequency threshold to $0$), 
the main purpose of our comparison is to examine trends in the runtime and stream-rate of each model using settings where they return comparable sets of subgraphs.
% TODO Discuss how we chose GraMi's (and GraphZip's) parameters
%In choosing \system{GraMi}'s parameters, we 
% Additional (theoretical) limitation for if the system were to run out of memory
% e.g. (1) if you actually tried to use GraMi to analyze a dynamic graph, you would have to store snapshots
% (2) depending on your systems RAM, the graph may be so big is can't be loaded into memory ("planet-scale" graphs)
% "To demonstrate this, we ran GraMi and GraphZip on the X dataset (10GB) on a 
% In contrast, GraphZip only needs enough memory for (a) dictionary and (b) current batch of edges at any point in time

Our results show that \system{\name} is clearly more scalable than \system{GraMi} when mining large graphs in the streaming setting. While processing \emph{NBER}, \system{GraMi}'s runtime (figure \ref{fig:graphzip_grami_rt_nber}) grows exponentially, experiencing a large spike near iteration 300. Figure \ref{fig:graphzip_grami_sr_nber} (normalized by 
%the number of 
patents per month) demonstrates this clearly: \system{\name} maintains a constant stream-rate throughout, while \system{GraMi}'s stream-rate gradually slows until it sharply drops near the final updates. In fact, \system{\name}'s stream-rate  shows a slight increase over time; one explanation is that as the captured patterns in $P$ become more complex, less isomorphism checks occur per batch.

Results on the \emph{HetRec} dataset indicate similar trends, though to a more extreme degree. With \emph{HetRec}, we use a minimum frequency threshold of 9,000 for \system{GraMi} and keep the previous settings for \system{\name}: setting the threshold to 1,000 causes GraMi's stream-rate to slow to a relative crawl, and when using 10,000, \system{GraMi} is able to process the entire dataset but only returns two frequent subgraphs. While processing \emph{HetRec} with the threshold set to 9,000, \system{GraMi} maintains a high stream-rate which trends upwards over time until the 93rd iteration, where the system freezes and is unable to make any progress despite being left running for multiple days (as indicated by the red `X' on figures \ref{fig:graphzip_streamfsm_sr_hetrec_l} and \ref{fig:graphzip_streamfsm_rt_hetrec_nl}). % TODO talk about why the constant stream-rate is so important!

% \vspace{-4mm}
\subsection{Comparison with \system{StreamFSM}}

Since there are no algorithms for mining highly-compressing subgraphs from graph streams in the existing literature, we benchmark \system{\name} against \system{StreamFSM}, a recently developed streaming algorithm for frequent subgraph mining. 
Subgraphs that compress well are often both frequent and large, so the tasks of mining highly-compressing and frequently-occurring subgraphs are closely related. 
%One weakness of the \system{StreamFSM} implementation is that it requires graph files be partitioned into batches before running the program, whereas \system{\name} will process with a constant batch size regardless of the file size. 
The \system{StreamFSM} reference implementation available online was unable to find any frequently occurring subgraphs with any large datasets other than the provided \emph{HetRec} dataset (we hypothesize this is likely due to an implementation error), so we report results for \system{StreamFSM} on the HetRec dataset only.

% TODO Compare results on HetRec to GraphZip and GraMi
% Both GraphZip and StreamFSM perform better than GraMi
% But what about the quality of results returned by GraphZip v StreamFSM? Number of patterns? Size, frequency, compression value?
A reasonable amount of time in the streaming setting equates to processing time less than or equal (at the very most) to the streaming-rate of the data; if the system cannot process the stream at the speed it is being generated, then the system is much less applicable in the real-life setting. Our results indicate that \system{\name} is significantly more scalable than \system{StreamFSM}: while \system{StreamFSM}'s stream-rate experiences an initial speedup, it quickly and consistently deteriorates after iteration 25, drastically increasing the runtime per iteration. The severe increase in runtime occurs around the same iteration that \system{GraMi} freezes (see figure \ref{fig:graphzip_streamfsm_rt_hetrec_nl}). In contrast, \system{\name} is seemingly unaffected by the same updates that cause massive slowdowns in \system{GraMi} and \system{StreamFSM}. \system{\name}'s stream-rate becomes relatively constant after an initial slowdown, and remains constant through to the end of the experiment (see figure \ref{fig:graphzip_streamfsm_sr_hetrec_l}). In the case of \system{\name} and \system{StreamFSM}, the stream-rate of both systems is much faster than the average stream-rate of the data ($7.8 \times 10^{-5}$ edges per second), despite \system{StreamFSM}'s relative volatility. However, a constant stream-rate is crucial for a deployed system processing a graph in real-time, since constraints on data processing time require predictable performance. % TODO expand on this

% \subsection{Efficiency Testing}
% In order to further demonstrate that \system{\name} scales linearly with the size of the graph (and that its stream-rate remains constant), we also test \system{\name} on the \emph{Delicious} user-tag network. TODO or CUT.

% \begin{figure*}[t]
% \begin{minipage}[t]{0.45*0.5\linewidth}
%     \includegraphics[width=\linewidth]{figures/graphzip_v_grami_streamrate_per_file_nber_lscale.pdf}
% %     \captionsetup{justification=raggedright}
%     \caption{
%     \system{GraphZip} stream-rate while processing \textit{NBER}. Higher is better.
%     }
%     \label{fig:graphzip_grami_sr_nber}
% \end{minipage}%
%     \hfill%
% \begin{minipage}[t]{0.45\linewidth}
% 	\centering
%     \includegraphics[width=\linewidth]{figures/graphzip_v_grami_runtime_per_file_nber_lscale.pdf}
%     \caption{\system{GraphZip} and \system{GraMi} runtime on \textit{NBER}.}
%     \label{f2}
% \end{minipage} 

% \begin{table}
%   \caption{\system{\name} vs \system{StreamFSM} runtime on the HetRec dataset. For reference, the average stream-rate of the HetRec dataset is $7.8 \times 10^{-5}$ (stream-rate is in units edges per second). We used the \system{StreamFSM} configuration with the best reported runtime in \cite{streamfsm} (frequency 500, 9 max-neighbors, gSpan frequence 0.1).}
%   \label{table:graphzip-streamfsm}
% %   \begin{center}
%   \begin{tabular}{@{}cccc@{}}
%   	\toprule
% 	Model & Parameters & Runtime (sec.) & Stream-rate (eps) \\
%     \midrule
%     \multirow{2}{*}{\name} & 50, 100 & 358 & 675.9 \\
%      & 100, 500 & 1634 & 148.1 \\
%     % & 500, 1000 & 1634 \\
% %     \midrule
%     \system{StreamFSM} & 500, 9, 0.1 & 2666 & 90.8 \\
%     \bottomrule
%   \end{tabular}
% %   \end{center}
% \end{table}

% \newpage

% \begin{figure}[t]
% \begin{minipage}[t]{0.45\linewidth}
%     \includegraphics[width=\linewidth]{figures/graphzip_streamrate_nber.pdf}
%     \caption{\system{GraphZip} stream-rate while processing \textit{NBER}.}
%     \label{f1}
% \end{minipage}%
%     \hfill%
% \begin{minipage}[t]{0.45\linewidth}
% 	\centering
%     \includegraphics[width=\linewidth]{figures/graphzip_v_grami_runtime_per_file.pdf}
%     \caption{\system{GraphZip} and \system{GraMi} runtime on \textit{NBER}.}
%     \label{f2}
% \end{minipage} 
% \end{figure}
% \clearpage
\begin{figure}[t]
\centering
   \begin{subfigure}{\columnwidth}
\includegraphics[width=\columnwidth]{figs-higgs_v_time.pdf}
\caption{Tracking Tweets per hour about the Higgs boson over time.}\label{fig:growth_higgs}
\end{subfigure}

\begin{subfigure}{\columnwidth}
\vspace{2mm}
% \includegraphics[width=\columnwidth]{higgs_sr.pdf}
\includegraphics[width=\columnwidth]{figs-higgs_v_time_and_sr.pdf}
\caption{Stream-rate of \system{\name} on the \emph{Higgs} dataset (higher is better).}\label{fig:sr_higgs}
\end{subfigure}
\vspace{-1mm}
\caption[]{(a) A large spike in activity occurs in the network after about 80 hours after the first Tweet. (b) After an initial slowdown, \system{\name} converges to a constant stream-rate.}
% \vspace{-1.7mm}
\end{figure}

\section{Twitter \& the Higgs boson particle}

% \begin{figure}[b]
% \includegraphics[width=\columnwidth]{figures/higgs_v_time.pdf}
% \caption{Tracking Tweets per hour about the Higgs boson over time. A large spike in activity occurs in the network after about 80 hours after the first Tweet.}\label{fig:growth_higgs}
% \end{figure}

% \begin{figure}[b]
% \includegraphics[width=\columnwidth]{higgs_tweets.pdf}
% \caption{Tracking Tweets per hour about the Higgs boson over time. A large spike in activity occurs in the network after about 80 hours after the first Tweet.}\label{fig:growth_higgs}
% \end{figure}

% \begin{figure}[b]
% \includegraphics[width=\columnwidth]{higgs_sr.pdf}
% \caption{Stream-rate of \system{\name} on the \emph{Higgs} dataset (higher is better). After an initial slowdown, \system{\name} converges to a constant stream-rate.}\label{fig:sr_higgs}
% \end{figure}

One weakness of the datasets analyzed in the previous sections is the low granularity of their timestamps, e.g., \emph{HetRec} can only be split into real-time streaming units as small as year, and the synthetic datasets have no time information at all. % (instead it must be arbitrarily sliced into streaming files). While we consider the flow-rate of the data (edges per interval time).
Streaming intervals (and therefore time between results) as long as a year are unlikely in a real deployment setting, especially when disk space is taken into consideration (storing a year's worth of data before processing largely negates the benefit of streaming). For example, given a graph mining system configured to mine activity from a live network such as Twitter, it is likely that the user(s) would configure the interval to analyze patterns and trends over days, hours or even seconds. Additionally, reducing the time period between batches can reveal ebbs and flows in network activity that would be hidden by averaging out activity over a longer period.

The \emph{Higgs}'s dataset has time data in seconds for each interaction, so we are able to pre-process the dataset into graph files segmented by the hour.
%(using a smaller time period would result in empty files). 
One benefit to using the \emph{Higgs} dataset is to observe how large spikes in network traffic affect the stream-rate; the minimum, maximum, and average number of edges streamed per hour are 43, 45,861, and 3,352 respectively, with the peak number of tweets per hour coinciding with the official announcement of the discovery.% (see figure \ref{fig:growth_higgs}).

As we can see in figure \ref{fig:sr_higgs}, \system{\name}'s stream-rate is unaffected by the large spike in network traffic (using the same model parameters as the previous experiments). After an initial slowdown (similar to \emph{HetRec}), \system{\name}'s stream-rate converges on a constant stream-rate slightly faster than the maximum stream-rate the network reaches at the 80 hour mark, and much faster than the average stream-rate of the network ($9.3 \times 10^{-1}$ tweets per second). Our results indicate that if \system{\name} had been deployed to monitor the graph stream in real-time, it would have been able to process each set of updates before the next set of updates arrived.

%Figure \ref{fig:patterns} shows two highly-compressing substructures mined from the dataset. Pattern A connects one user to seven others via retweets (the red nodes retweet the yellow nodes). Pattern B is slightly more complex, but also maintains the star pattern as its core structure. The yellow node represents an initial tweet, which then cascades through the network as `mentions' (blue nodes), apart from a single user who retweets the post.

% \begin{figure}[t]
% \includegraphics[width=\columnwidth]{figures/patterns_higgs_3.png}
% \caption{Two highly-compressing patterns in the pattern dictionary from processing the \emph{Higgs} dataset. Pattern A shows several users that are found to consistently \emph{retweet} node (user) $u_1$ simultaneously, while pattern B shows a frequently occurring cascade of interactions as \emph{mentions} (originating at $u_1$) throughout a cluster of nodes.}
% \label{fig:patterns}
% \end{figure}


%% 1-2 paragraphs
\section{Conclusion and Future Work}
In this paper, we introduced \system{\name}, a graph mining algorithm that utilizes a dictionary-based compression approach to mine highly-compressing subgraphs from a graph stream. 
%To the best of our knowledge, \system{\name} is the first system f,
We showed that \system{\name} is able to successfully mine artificially-generated graphs for maximally-compressing patterns with comparable accuracy and much greater speed than a state-of-the-art approach. Additionally, we also demonstrated that \system{\name} is able to surface both complex and insightful patterns from large real-world graphs at speeds much faster than the actual stream-rate, 
%a computationally intractable task for non-streaming methods. 
with performance exceeding that of openly available state-of-the-art non-streaming and streaming methods. Future work will focus on implementing the potential optimizations to the algorithm discussed in this paper, including approximation algorithms for (subgraph) isomorphism computations and na\"{\i}ve parallelization.


\appendix
%Appendix A
% TODO Add space complexity?
\section{Complexity Analysis}
In this section we examine the time complexity of algorithm \ref{alg:graphzip} 
%(\system{\name}) 
in detail. We begin by analyzing the runtime per batch $B$ from a stream of graph $G$. Given a batch $B$, for each pattern $P^{(i)} \in P$ we retrieve the set $M$ of all embeddings (subgraph isomorphisms) of $P^{(i)}$ in $B$:
\begin{equation} \label{e.c1}
 \mathcal{O}(|P| \times \mathcal{O}(SI(P^{(i)},B)))
\end{equation}
Then, for each embedding $M^{(i)} \in M$, we (a) extend a copy of $M^{(i)}$ by one edge length in each direction and (b) add the new pattern to the dictionary:
\begin{equation} \label{e.c2}
\begin{aligned}
\mathcal{O}(&|P| \times (\mathcal{O}(SI(P^{(i)},B))\ + \\
& |M| \times (|V_{M^{(i)}}| \times k + |P| \times \mathcal{O}(I(M^{(i)'},P^{(i)})))))
\end{aligned}
\end{equation}
where $k$ is the number of edges incident of $v \in V_B$ shared with $u \in V_{M^{(i)}}$, and $M^{(i)'}$ is the extended copy of $M^{(i)}$. Finally, we add the remaining edges in $B$ as single-edge patterns ($e$) to $P$:
\begin{equation} \label{e.c3}
\begin{aligned}
\mathcal{O}(&|P| \times (\mathcal{O}(SI(P^{(i)},B))\ + \\
&|M| \times (|E_{M^{(i)}}| \times k + |P| \times \mathcal{O}(I(M^{(i)'},P^{(i)}))))\ +\\
&|R| \times \mathcal{O}(I(e,P^{(i)})))
\end{aligned}
\end{equation}
If we use the well-known VF2 algorithm to implement the subgraph and graph isomorphism functions, the time complexity for $SI(.)$ and $I(.)$ simplify to $\mathcal{O}(V^2)$ in the best case and $\mathcal{O}(V! \times V)$ in the worst case, where $V$ is the maximum number of vertices between the two graphs. Recall that our model is parameterized by $\theta$ and $\alpha$ ($|P|$ and $|E_B|$ respectively), which directly bounds $k < |V_B| < 2\alpha$, $|M| < 2^{\alpha}$ (maximum number of possible subgraphs in $B$), $E_{M^{(i)}} < \alpha$, and $|R| < \alpha$. Substituting into the worst case using VF2, we get:
%TODO explain where the 2! * 2 constant comes from
% Explain why |B_V| < 2\alpha ?
\begin{equation} \label{e.c4}
\begin{aligned}
\mathcal{O}(&\theta \times (({(2\alpha)! \times 2\alpha)} \ + \\
&2^{\alpha} \times (\alpha \times 2\alpha + \theta \times {((2\alpha)! \times 2\alpha)}))\ +\\
&\alpha \times 2! \times 2)
\end{aligned}
\end{equation}
Which simplifies to:
\begin{equation} \label{e.c5}
\begin{aligned}
\mathcal{O}(&\theta \times \alpha! \times \alpha \ + \\
&\theta \times(2^{\alpha} \times \alpha^2 + 2^{\alpha} \times \theta \times \alpha! \times \alpha) +\\
&\theta \times \alpha)
\end{aligned}
\end{equation}
And lastly:
\begin{equation} \label{e.c6}
\mathcal{O}(\theta^2 \times 2^{\alpha} \times \alpha! \times \alpha)\\
= \mathcal{O}(\theta^2 \times \alpha!)
\end{equation}
% \begin{equation} \label{e.c7}
% \mathcal{O}(\theta^2 \times \alpha!)
% \end{equation}

Since $\theta$ and $\alpha$ are provided as parameters (constants at run-time), eq. \ref{e.c6} theoretically collapses to constant time ($\mathcal{O}(1)$), meaning that the \system{\name} algorithm scales linearly with the size of the overall graph. However, our complexity analysis illustrates an important trade-off in selecting the batch size and dictionary size, since too large a value for either parameter can exponentially increase the run-time per batch (increasing \batchsize{} is particularly costly).

Our theoretical complexity analysis reinforces our experimental findings: that subgraph isomorphism calculations (a known NP-complete problem) dwarf all other computations in the algorithm. A promising area of future work would be to incorporate existing approximation algorithms for the subgraph isomorphism problem to increase the efficiency of \system{\name}.

% TODO expand (specifically) on how this would change the run-time

\begin{acks}
This material is based upon work supported by the \grantsponsor{}{National Science Foundation}{} under Grant No.:~\grantnum{}{1460917} and~\grantnum{}{1646640}.
% We thank Abhik Ray for generously providing a reference implementation of \system{StreamFSM}.

%   The authors would like to thank Dr. Yuhua Li for providing the
%   matlab code of  the \textit{BEPS} method. 

%   The authors would also like to thank the anonymous referees for
%   their valuable comments and helpful suggestions. The work is
%   supported by the \grantsponsor{GS501100001809}{National Natural
%     Science Foundation of
%     China}{http://dx.doi.org/10.13039/501100001809} under Grant
%   No.:~\grantnum{GS501100001809}{61273304}
%   and~\grantnum[http://www.nnsf.cn/youngscientsts]{GS501100001809}{Young
%     Scientsts' Support Program}.
\end{acks}

